Symplectic and Poisson geometry of the information geometry's Frobenius manifold

We prove that the information geometry's Frobenius manifold is a symplectic manifold having Poisson structures. By proving this statement, a bridge is created between the theories developed by Vinberg, Souriau and Koszul and the Frobenius manifold approach. Until now these approaches seemed disconnected.

==> Symplectic arXiv/Hamiltonian.tex <==
\subsubsection{Recollections on the construction of the Hamiltonian system}
For the convenience of the reader, some recollections are presented (in this subsection) in relation to the Hamiltonian system.
%State phase/ configuration space 
Let $M$ be a manifold of dimension $n$ and let $x=(x^1,...,x^n)$ be the canonical coordinates attached to a point $x$ on $M$. %corresponding to the position, in the phase space. In our case, this will correspond to the fourth Frobenius manifold. 
We construct a Hamiltonian system using the $2n$-dimensional fibered cotangent bundle $T^*(M)$.
Given a point $x\in M$ and a covector $p=(p_1,...,p_n)$ attached to $x$, we have the following closed (and exact) differential form given by:
\[ \sum_{\alpha}dx^{\alpha}\wedge dp_{\alpha}.\]

\smallskip 

Note that the differential form $\Omega=d\omega,$ where $\omega$ is given by $p_{\alpha}dx^\alpha$ is defined globally on $T^*(M)$ if and only if the form is {\it proportional} to the volume element (with a non-nul proportionality coefficient). In particular, this form defines the scalar product (alternate and non-degenerate) of a pair of vectors:
\[\langle \xi, \eta \rangle=-\langle \eta, \xi\rangle=J_{ij}\xi^i\eta^j \]
where $i,j=1,2,...,2n;$\, $\Omega=J_{ij}dy^i\wedge dy^j$, with non-nul $J_{ij}$ and $(y^1,\dots,y^{2n})$ are canonical coordinates on $T^*(M)$ given by:

\[y^i=x^i \quad y^{n+i}=p_{i},\quad i=1,2,...,n.\]
Using this, we establish a relation to phase space (in the physics setting) and therefore to configuration spaces of marked points in the euclidean space.


Now, this leads to the Hamilton equation:

\[\frac{dy}{ds}=J^{ij}\frac{\partial \mathcal{H}}{\partial y^j}, \quad J^{ij}J_{jk}=\delta_{k}^{i}.\]
where $s$ is a real parameter.

%\subsection{The Hamiltonian}

We present the explicit construction of the Hamiltonian for the case of the information geometry's $F$-manifold. 
As it is known, the energy $\mathcal{E}$ is given by $\mathcal{E} = \mathcal{H}(x, p)$ where  
\[\mathcal{H}(x, p) = \frac{1}{2} \langle p\, ,\, p \rangle,\]
and $p$ was defined above. 

Since $p$ can be considered as a linear operator, given by $\frac {\partial }{\partial x}$
then the Hamiltonian can be written as a bi-linear form:
 $\mathcal{H} (x\, ,\, \frac{\partial}{\partial x})=\mathcal{H}(x\, ,\, \xi)$. This corresponds to the 2- form: $\langle\frac {\partial}{\partial x}\, ,\, \frac{\partial}{\partial x}\rangle=\langle\xi\, ,\, \xi\rangle.$
In the following we show an explicit Hamiltonian for the information geometry fourth Frobenius manifold. 
%%%AMARI


==> Symplectic arXiv/PoissonBrackets.tex <==
\section{Poisson structures}
In this section, we present the Poisson bracket for the information geometry $F$-manifold. We consider a symplectic manifold. Novikov, in his works on symplectic geometry, introduced a special type of Poisson brackets for this type of manifold. More specifically, we called them the {\it Novikov--Poisson brackets}. Initially, these Novikov--Poisson brackets were introduced to construct a theory of conservative systems of hydrodynamic type. It strongly interferes in the existence of Frobenius manifold structure.


By the previous section, we have the following  proposition:

 \begin{prop}
The information geometry fourth Frobenius manifold  is a symplectic (paracomplex) manifold $(M,\Omega_{\frak{C}},\Omega)$ with the 2-form $\Omega_{\frak{C}}=\frac{e}{2}g_{jk}dz^j\wedge d\overline{z}^k,$ where $e^2=1$ and $g_{jk}$ is a paracomplex bilinear form and $\Omega=dz^j\wedge dp_k.$
\end{prop}

This can be enlarged to Poisson structures and Poisson manifolds.  A Poisson structure is a Lie algebra bracket $\{\cdot\,,\, \cdot\}$ on the vector space of smooth functions on a manifold $M$ which form a Poisson algebra with the point-wise multiplication of functions. Therefore, we can say that:
\begin{cor}
The information geometry fourth Frobenius manifold carries a Poisson structure and thus is a Poisson manifold. 
\end{cor}

The Poisson bracket on the paracomplex space $\{\cdot\, ,\,\cdot \}_{\frak{C}}$ is given by \[\{\xi,\eta\}_\frak{C}=\frac{1}{2}Im \langle \xi,\eta \rangle_{\frak{C}}=\frac{e}{2}\left(\frac{\langle \xi, \eta \rangle_{\frak{C}}- \overline{\langle \xi, \eta \rangle_{\frak{C}}}}{2}\right),\] where $e$ satisfies $e^2=1$ and $Im$ is the imaginary part of a paracomplex number. 

We consider this Frobenius manifold as a certain type of phase space, i.e. $(z^1,\cdots, z^n,\, p_1,\cdots, p_n, \Lambda_1,\cdots, \Lambda_m)$,
where the $z^\mu$ are paracomplex numbers, $p_\mu=p_\mu(z)$ are 1-forms of the fibered cotangent bundle attached at the point $z$ and the $\Lambda_i$ are $m$ functions on the phase space. For instance, concerning the set of functions $\{\Lambda_i\}_{i=1}^m$ on the phase space we can consider them as a set of spins of Ising, Heisenberg or any other relevant structure. In the case of the Ising spin model we have $m=1$. Whereas, for the case of the Heisenberg model $m=3$.

\smallskip 

The set $\{\Lambda_i\}_{i=1}^m$ can have a Lie algebra structure, if the Poisson bracket of a pair of functions $\Lambda_i$ and $\Lambda_j$ is obtained by a linear combination of those functions, for $i,j\in \{1,\cdots,m\}$. More precisely, we have $\{\Lambda_i,\Lambda_j\}=-\Lambda_k\gamma^k_{ij}$, where $\gamma^k_{ij}$  are structure constants of the algebra. 

Let $A, B$ be a pair of functions on the phase space $(z^1,\cdots, z^n,p_1\cdots, p_n)$. These are observables and can be for example the momentum. $A$ and $B$ are real functions depending on $z$ and $p$. Then, the Poisson bracket is given by:
\[\{A,B\}=\frac{\partial A}{\partial p_\mu}\frac{\partial B}{\partial z^\mu}-\frac{\partial B}{\partial p_\mu}\frac{\partial A}{\partial z^\mu}.\]

The Poisson bracket can be interpreted as a type of derivation on the functions $A$ and $B$ in the sense that for any given pair of smooth phase functionals $f(A)$ and $g(B)$ we have the following relation:

\[\{f(A),g(B)\}=f'(A)g'(B)\{A,B\}.\]
In the generalised context, i.e. for $A=(A_1,\cdots, A_r)$ and $B=(B_1,\cdots B_l)$ we have:
\[\{f(A),g(B)\}=\frac{\partial f}{\partial A_i}\frac{\partial g}{\partial B_j}\{A_i,B_j\}.\]

\begin{rem}
Note that the derivation of smooth functions correspond to smooth tangent vector fields (for every given smooth function). So, for a smooth function $f$ there exists a vector $X_f$ given by $X_f(g)=\{f,g\}$. This is also known as the {\it Hamiltonian vector field}, corresponding to the function $f$. 
\end{rem}



In the most general setting, that means in the generalised phase space where the $\Lambda_i$ functions enter the game, $(z^1,\cdots, z^n,\, p_1,\cdots, p_n, \Lambda_1,\cdots, \Lambda_m)$ we have the Poisson bracket defined as:
\[\{A,B\}=\frac{\partial A}{\partial p_\mu}\frac{\partial B}{\partial z^\mu}-\frac{\partial B}{\partial p_\mu}\frac{\partial A}{\partial z^\mu}-\Lambda_k\gamma^k_{ij}\frac{\partial A}{\partial \Lambda_i}\frac{\partial B}{\partial\Lambda_j}.\] 

Note that for an arbitrary Hamiltonian $\mathcal{H}(p,z,\Lambda,s)$ and a smooth phase space function $Q(p,z,\Lambda)$ the equation of motion is described by $\dot{Q}=\frac{dQ}{ds}=\{\mathcal{H},Q\}.$ This is identified to the notion of a {\it symplectic gradient}. Indeed, a symplectic gradient is
a unique vector field $X_{\mathcal{H}}$ described by the condition $X_{\mathcal{H}}(Q)=\{\mathcal{H},Q\}$. For instance, one can write the following symplectic gradient: $X_{\mathcal{H}}(z^\mu)=\frac{d z^\mu}{ds}= \{\mathcal{H},z^\mu\}$ where $\mathcal{H}$ is the Hamiltonian, mentioned and constructed in the above section. More formally, the symplectic gradient of $\mathcal{H}$ is the vector field given by:
\[X_{\mathcal{H}}:=\Omega_{\frak{C}}^{-1}d_{dR}\mathcal{H},\]
where the symbol $d_{dR}$ is the {\it de Rham differentia}l, mapping smooth functions on $M$ to 1-forms on $M$. On the fiber bundle space $T^*(M)$, we can indeed define a symplectic gradient. Since the 2-form $\Omega_{\frak{C}}$ is closed, the Poisson brackets introduce on the linear space of functions a Lie algebra structure. 

%\[\begin{cases}
% \frac{d z^\mu}{ds}= &\{\mathcal{H},z^\mu\}\\
%$  \frac{d p_\mu}{ds}= &\{\mathcal{H},p_\mu\}
% \end{cases}\] 
 


%\[f\mapsto \nabla f=\{A_i,B_j\}\frac{\partial f}{\partial A^j},\]\[g\mapsto \nabla g= \{A_i,B_j\}\frac{\partial g}{\partial B^j},\]
%so \[\{f,g\}\to [\nabla f, \nabla g].\]
%(For more information, see p.281 in~\cite{DNF}.)

We have thus the important corollary,  that the fourth Frobenius manifold is a Poisson manifold and is thus extensively equipped with Poisson Geometry. 

\smallskip 

The following discussion, tends to show a connection of our latter statement with the works in~\cite{Ba20}. In particular, our last statement establishes a bridge to the works of Koszul--Souriau \cite{Ba16,Ba20,Ko,Sou65}. 



The Frobenius structure is closely related to the Poisson bracket of hydrodynamic type (see \cite{BaNo,DuNo}). More precisely, we present the definition of Poisson bracket of hydrodynamic type and discuss the consequences. 

We define the Novikov-type of Poisson bracket, based on the works of~\cite{BaNo,DuNo}. 

\begin{defn} The Novikov--Poisson bracket is a Poisson bracket of hydrodynamic type, defined by the following equation:
 \begin{equation}\label{E:p}
  \{u^i(x),u^j(y)\} = g^{ki,\alpha}(u(x))\partial_\alpha\delta'(x - y) + b^{ki,\alpha}_j(u(x))\partial_\alpha u^j\delta(x - y),\end{equation} 
  where $u^j$ are fields (usually the density of momentum and energy or mass) and $b^{ij}_k$ is a tensor. 
\smallskip 
 \end{defn}
 
Remark the following. 
\begin{lem}
Let $z=(z^1,\cdots,z^n)$ and $w=(w^1,\cdots,w^n)$ be two points on a paracomplex manifold and let $u(z)=(u^1(z),\cdots, u^n(z))$, $v(w)=(v^1(w),\cdots, v^n(w))$ (with $u^i(z)=u(z^i)$) be two ''observables'' on the phase space, associated to the paracomplex Frobenius manifold. 
Then, $\{u^i(z)\, ,\, u^j(w) \}=g^{ij}(u(z)\delta'(z-w))+\frac{\partial u^k}{\partial z}b^{ij}_{k}(u(z)\delta(z-w))$.
\end{lem}
\begin{proof}This follows from the discussion in section 2 on paracomplex spaces, from the result in\cite{CoMa20} showing the existence of paracomplex geometry of the fourth Frobenius manifold and from \cite{DuNo}.\end{proof}
%Note that this expresses the 2-dimensional case. A generalisation to higher dimensions is possible. However, for simplicity we choose not to write it.
\smallskip 

The classification of Poisson brackets has been done in (\cite{BaNo}). This classification depends linearly on $u^k$ and is relative to linear changes $u^k = A^k_j w^j$. It can be obtained through the classification of Lie algebras and Frobenius algebras. Indeed, the {\it simplest local Lie algebra} arises from the brackets as follows: 

\[g^{ij}=C^{ij}_ku^k+g_{0}^{ij}, \quad b_k^{ij}=\text{cst}, \quad g_{0}^{ij}=\text{cst};\]
\[ [p,q]_k(z) = b^{ij}_k(p_i(z)q_j'(z)- q_i(z)p'_j(z))\]
 where 
 \begin{equation}\label{E:b}
  b^{ij}_k+b^{ji}_k=C^{ij}_k=\partial g^{ij}/\partial u^k.
  \end{equation} 
 \begin{rem}
It is precisely the tensor $b^{ij}_k$ (from equation\, \eqref{E:b}) which plays an important role from the side of the Lie algebra. Indeed, it defines a local, translationally invariant Lie algebra of first order, if and only if the following condition is fulfilled. 
\begin{center}
{\bf Condition:} {\it The tensor $b^{ij}_k$ plays the role of the constant structure in the multiplication law of a finite dimensional algebra $\mathcal{A}$ defined by the identities:}
 \smallskip 
 
\[a,b,c\in \mathcal{A},\quad e^ie^j\quad e^ie^j=b_k^{ij}e^k;\]
\[a(bc)=b(ac),\quad (ab)c-a(bc)=(ac)b-a(cb).\] 

\end{center}

The algebra $\mathcal{A}$ is associative and commutative if the condition $2b_{ij} = 2b_{ji} = C_{ij}$ is fulfilled. By definition, this algebra is called Frobenius if there exists a given  non-degenerate inner product satisfying the associativity condition i.e. such that: $\langle e_i\circ e_j\, ,\, e_k \rangle=\langle e_i\, ,\, e_j\circ e_k \rangle.$ The necessary
and sufficient condition for an algebra with identity such as $\mathcal{A}$ to be Frobenius is that $2b_{ij}u^k = C_{ij}u^k$ is {\it non-degenerate} at a generic point. 

\smallskip  
Let us explicit our thought. The $b^{ki,\alpha}_j$ (resp. $b_{ji}^k$ in a less general context) plays a decisive role, regarding the Frobenius structure in the following way. Those tensors correspond to the constant structures in the multiplication law of the Frobenius algebra $\mathcal{A}_p$, associated to the Frobenius manifold $M$. More precisely, the Frobenius algebra is associated to the tangent space of a Frobenius manifold $T_pM$, at a given point $p$. This leads to the formulation of the statement below.  

\begin{lem}
For the information geometry's Frobenius manifold, there exist Poisson brackets of hydrodynamic type, (equation \eqref{E:p}) such that the tensors $b^{ij}_k$ correspond to the constant structures in the multiplication law of the Frobenius algebra, associated to the tangent space to the Frobenius manifold.
\end{lem}
\begin{proof}
This follows from the definition of Frobenius manifold introduced by Dubrovin in~\cite{Du96} and from the principal statement in~\cite{BaNo}. 
\end{proof}
In particular, we have the following statement:

\begin{lem}
Let $(M,\Omega)$ be the symplectic information geometry Frobenius manifold. Then, the phase space associated to it has an algebraic structure depending on the tensors $b^{ki,\alpha}_j$, defined in equation \eqref{E:p}. 
\end{lem}
\begin{proof}
Let us map $T_pM$ to its dual space $T^*_pM$ by a linear operator $\Phi$. Then, there exists a map $\tilde{\phi}:\mathcal{A}_p\to \mathcal{A^*}_p$, where    $\mathcal{A^*}_p$ is the algebra attached to $T^*_pM$. Following the commutative diagram below, we have that $\tilde{\phi}=\Psi^{-1}\circ\Phi\circ\chi$ is a homomorphism.
\[
\begin{tikzcd}
\mathcal{A}_p \arrow{r}{\tilde{\phi}} \arrow[swap]{d}{\chi} & \mathcal{A^*}_p \arrow{d}{\Psi} \\
T_pM  \arrow{r}{\Phi} & T^*_pM
\end{tikzcd}
\]



Therefore, by duality (and only for finite dimensional cases!) the $b^{ki,\alpha}_j$ are the constant structures of the algebra associated to the cotangent space $\mathcal{A^*}_p$. So, the coefficients $b^{ki,\alpha}_j$ determine the underlying algebraic structure of the phase space and thus of the symplectic paracomplex manifold. 

\end{proof}

\smallskip 

Finally, one last remark concerning the Poisson geometry of this Frobenius manifolds. The  Novikov--Poisson brackets  (hydrodynamic type) are tightly related to the metric of the manifold in the following way. 

\begin{prop}
On the fourth Frobenius manifold, there exist flat pencils of Koszul--Souriau metrics, being related to compatible Novikov--Poisson brackets.
\end{prop}
\begin{proof}
Suppose we have a flat metric in some coordinate system $\{x^i\}$. If the components of the metric $g^{ij}(x)$ and the Christoffel symbols $\Gamma^{ij}_k$ of the corresponding Levi--Civita connection depends linearly on the coordinate $x^1$, then the metrics form a {\it flat pencil:} 

\[g^{ij}\quad \text{and}\quad  g_2^{ij}:=\partial g^{ij}\]

(it is assumed that the determinant of $g_2^{ij}$ is not zero). 

A pair of Poisson brackets  (hydrodynamic type) $\{\cdot\, ,\, \cdot\}$ are called {\it compatible} if an arbitrary linear combination with constant coefficients of those brackets defines back a Poisson bracket. Flat pencils of metrics correspond to {\it compatible pairs of poisson brackets} (hydrodynamic type) (see \cite{Du96}). Therefore, we have the existence of flat pencils of Koszul--Souriau metrics for the fourth Frobenius manifolds.
\end{proof}

\smallskip 


\section{Remarks}
We can remark the following facts. 
\begin{rem} Orbits (that means geodesics) in the fourth Frobenius manifold are given by some trajectories given in paraholomorphic coordinates. 
Motions along these paraholomorphic orbits are {\it non dissipative}~\cite{NeSe}. In particular, by non dissipative motion we mean that  the production of entropy (during the motion) is null. In the latter case---and referring to Souriau's theory---we have an equality between the inner statistical states and the outer statistical states. Whereas the motion of transversal vectors to these surfaces is dissipative \cite{Ba20,BuNePe}.
\end{rem}

 \end{rem}
 \begin{rem} 
The orbit (that means a given geodesic) on a paracomplex space is decomposed into two orbits. Following the construction of paracomplex spaces defined in section 2, each of these orbits lies on a flat submanifold, corresponding respectively to one of the generators: $e_+$ or $e_-$ of the algebra. These two orbits are equidistanced to the {\it Peirce mirror}. 

\smallskip 

We digress on the notion of Peirce reflection (or Peirce mirror) for the convenience of the reader.  Peirce reflections arise for a given unital Jordan algebra (say $J$) with orthogonal idempotents $a, a'$ i.e. verifying the condition $a a'=a'a=0$. We are precisely in this case (see~\cite{CoCoNenFICC}).  
Considering a pair of orthogonal idempotents $a, a'$ and by putting $u=a-a'$ we can show that $u$ is an involution. Now, 
if $u$ is an involution in a unital Jordan algebra $J$, then one can define an involutionary automorphism of $J$, i.e. $U_u^2 = 1_J$ (see lemma 6.10 in \cite{MC04}). Then this involution has a description as a Peirce reflection in terms of the Peirce projections (see p.238 \cite{MC04} for more details). For further details and relations between the fourth Frobenius manifold and Peirce's reflection and decomposition theorems, see \cite{CoCoNenFICC}.

\smallskip 

In the light of the Peirce mirror, we can say that these orbits form a so-called pair of Clifford parallels. By Clifford parallel we mean a straight line in an elliptic space staying at constant distance from a given base (straight) line. The motion on paraholomorphic orbits is equivalent to the motion on pairs of Clifford parallels. Using the previous remark, we can state that the paraholomorphic motion of Clifford pairs is non dissipative. 
\end{rem}


%It is important to note that from the perspective of Morozova--Chentsov~\cite{} (equation 7.3) one can explicitly outline a bilinear form, corresponding to the Hamiltonian. This statement is summarized in the following lemma.

%\begin{lem}
%There exists a 2-form on the finite dimensional paracomplex space corresponding to the finite space of probability distributions such that:
%For the Morozova--Chentsov information geometry framework, there exists a 2-form 
%\begin{equation}\label{E:2}%7.3
%\sum u^{ik}\xi^i\xi^k+2\sum v^{ik} \xi^i \eta^k +\sum w^{ik}\eta^i \eta^k,
%\end{equation}
%where $u, v, w$ are the coefficients of the polar bilinear form and form the components of $g_{ij}$  the metric tensor for the paracomplex numbers.
%\end{lem}
%$\xi$ (resp. $\eta$), are respectively the real and imaginary parts of a paracomplex vector and are in one to one correspondence with a probability distribution $P$ (resp. $Q$). An intuition of this had started to dawn in the works of Morozova--Chentsov  \cite{MoChen}. However, the construction relating the paracomplex space and the space of probability distributions follows from~\cite{CoMa20}. Further details concerning this are thus omitted. 
%\begin{equation}%7.3
%\sum u_{jl}^{ik}\xi_j^l\xi_l^k+2\sum v_{jl}^{ik} \xi_j^i \eta_l^k +\sum w_{jl}^{ik}\eta_j^i \eta_l^k,
%\end{equation}
%The 2-form given in \eqref{E:2} corresponds to the form $\Omega$, discussed previously.


==> Symplectic arXiv/S1IntegrableSystem.tex <==
\section{Proof of the main theorem}

We expose the proof of the main theorem. It is known that a symplectic manifold is an integrable system, equipped with a Hamiltonian action (for sinatance see \cite{Mo09}), relying on the metric tensor of the manifold. As was presented in the introduction, the discussion is decomposed into two principal steps:

\begin{itemize}
\item The fourth Frobenius manifold is an integrable system.
\item This integrable system is a Hamiltonian one, depending on the tensor metric of the manifold. Smaller steps are needed to prove this statement, (we choose not mention them here, for simplicity). Recollections on Hamiltonian systems and paracomplex geometry are needed for the reader's convenience. 
\end{itemize}
\medskip 
\subsection{First step: integrable system}
 To prove that we have an integrable system, we invoke the following theorem of Mokhov~\cite{Mo07,Mo09} stating that:

\smallskip 

{\it The class of flat, torsionless submanifolds in any Euclidean or pseudo-Euclidean space is an integrable system.}

\smallskip 


Now, we know from \cite{Du96,CoMa20,Man99} that the Frobenius manifold is necessarily {\it flat and torsionless}. Therefore, the information geometry fourth Frobenius manifold is an integrable system. This proves the first step. 

\medskip 

\subsection{Second step: Hamiltonian system} The second steps means that we ought to show that the system is a Hamiltonian one.
Namely, the important statement to use is that  the system {\it has} a Hamiltonian structure if and only if the {\it Lagrangian $\mathcal{L}$ depends on the tensor metric}, i.e. $\mathcal{L}(x,\xi)=g_{ij}(x)\xi^i(x)\xi^j(x) - U(x),$
where $x$ are canonical coordinates on the manifold, $g_{ij}$ is the tensor metric, $U$ is a scalar field and $\xi^i,\xi^j$ are vector fields. %The action is such that to a given point $x$, mapped to a tangent vector $\delta x$, the action is a functional of $x$ and the tensor metric $g_{ij}$
%\[A
\smallskip

%For instance, in the case of the first Frobenius manifold (i.e. Quantum cohomology, in the classification of Manin~\cite{MaF}) related to the $\sigma$-models, the action has a form given by: 
%%\[\int(\frac{1}{2}g_{ij}(\xi) \xi^i_x\xi^j_t-U(\xi))dxdt \longleftrightarrow g_{ij}(\xi)\xi_{xt}^d+g_{is}(\xi)\Gamma_{jk}^s(\xi)\xi_x^k\xi_t^j=\frac{\partial U}{\partial\xi^i},\]
%where $g_{ij}$ is an arbitrary (pseudo)-Riemannian metric in a given (target) Euclidean space $M$ with local coordinates $(\xi^1,\dots,\xi^n)$ and the functions $\xi^i(x,t)$ correspond---in the context of $\sigma$-models---to Bosonic fields (see~\cite{Mo07,Mo09}). 

\input{Hamiltonian}
\smallskip 
\subsubsection*{Hamiltonian construction for the fourth Frobenius manifold}
We continue by showing the explicit construction of the Hamiltonian. From~\cite{CoMa20}, it is known that the information geometry $F$-manifold has a {\it paracomplex structure}. It implies that the construction of differential forms for paracomplex  geometry is necessary. Therefore, we recall a few notions on paracomplex geometry. 

\smallskip 
\subsubsection*{Recollections on paracomplex geometry}
Let us define the rank 2 algebra of paracomplex numbers $\frak{C} = \mathbb{R} + e\mathbb{R}$. This is a split algebra, generated by the basis $\{1,e\}$ where $e^2=1$. It resembles the field of complex numbers in the sense that a paracomplex number $z=x+ey$ has a paracomplex conjugate $\overline{z}=x-ey$ where $e$ squares to +1. However, this algebraic structure does not form a field. On the other side, an interesting feature of this split algebra is that it has a {\it pair of idempotents}.

An idempotent $a$ in an algebra is element such that $a^2=a.$ In the algebra of the paracomplex numbers the pair of idempotents can be seen using a suitable change of basis. The new basis is generated by $e_{+}$ and $e_{-}$ where $e_{\pm}=\frac{1\pm e}{2}$. It can be easily checked that $e_+^2=e_+$ (resp. $e_-^2=e_-$). This pair of idempotents plays an important geometric role, since it implies the existence of a Peirce reflection (also known as Peirce mirror).   

\smallskip 

Let us roughly recall the notions of paraholomorphic structures and manifolds.  Denote by $E_{2m}$ a $2m$-dimensional real affine space. {\it A paracomplex structure} on $E_{2m}$ is an endomorphism $\frak{K}: E_{2m} \to E_{2m}$ such that $\frak{K}^2=I$,
and the eigenspaces $E_{2m}^+, E_{2m}^-$ of $\frak{K}$ with eigenvalues $1,-1$ respectively, have the same dimension. A {\it paracomplex manifold} is a real manifold $M$, equipped with a paracomplex structure $\frak{K}$, admitting an atlas of paraholomorphic coordinates---being functions with values in the split algebra of paracomplex numbers---and such that the transition functions are paraholomorphic.

\smallskip 

Considering a module over the paracomplex algebra, and more precisely its (real) realisation as a linear space, a domain $D$ in the paracomplex space contains paracomplex points $z=(z^1,\cdots,z^n)$, which are given by:

\[z^k=x^k+e y^k,\]

and by definition we have $e^2=1$ and $k\in \{1,\cdots,n\}$. 

\smallskip 

The existence of the paracomplex structure implies the existence of local coordinates $(z_+^\alpha, z_-^\alpha),\, \alpha = 1,\cdots, m$ such that
paracomplex decomposition of the local tangent fields is of the form
\[
T^{+}M=span \left\{ \frac{\partial}{\partial z_{+}^{\alpha}},\, \alpha =1,\cdots, m\right\},
\]
\[
T^{-}M=span \left\{\frac{\partial}{\partial z_{-}^{\alpha}}\, ,\, \alpha =1,\cdots, m\right\} .
\]
Such coordinates go by the name of {\it adapted coordinates} for the paracomplex structure $\frak{K}$.

The dual basis for the differential forms (dual basis to the paracomplex tangent vectors) is given by:

\[dz^k=dx^k+edy^k, \quad d\overline{z}^k=dx^k-edy^k,\quad k=\{1,\cdots,n\}.\] 

\smallskip 

Similarly to the complex case, we have a splitting of the differential forms:
\[d=d'+d'',\] where for a given $(p,q)$ paracomplex form $\omega$ the differential $d'\omega$ is a $(p+1,q)$-form, whereas $d''\omega$ is a$(p,q+1)$-form. It is easily seen that \[(d')^2=(d'')^2=0\] and that \[d''d'=-d'd''.\]

\smallskip 

In order to obtain the Hamiltonian on the paracomplex manifold, we introduce a local paracomplex Dolbeault (1,1)-form. This is given by:

\[\omega:=\partial_+\partial_-\phi\]
where $\phi$ is the potential function defined uniquely modulo subspace of local functions $ker \partial_+\partial_-$ and $\partial_\pm$ are given in canonical paracomplex coordinates. 

To show that the Hamiltonian relies on the metric tensor, it is sufficient to consider the scalar product on a space with paracomplex structure. By definition the scalar product is defined as:
\[\langle \xi, \eta \rangle_{\frak{C}}= g_{jk}\xi^j\overline{\eta^{k}}.\] 
This scalar product is a Hermitian one, since we have the equality:
\[\langle \xi, \eta \rangle_{\frak{C}}=\overline{\langle \eta,\xi \rangle_{\frak{C}}}.\]

 
Then, the paracomplex differentiable 2-form is given by: \[\Omega_{\frak{C}}=\frac{e}{2}g_{jk}dz^j\wedge d\overline{z}^k.\]

By definition, it is known that the Hamiltonian is a 2-form, so we have proved that a Frobenius manifold---with paracomplex structure---is an integrable system with Hamiltonian.  

\medskip 
\subsection{The symplectic fourth Frobenius manifold}
It remains to adapt this construction to the information geometry Frobenius manifold. 

%\begin{lem}
%The information geometry fourth Frobenius manifold  is a symplectic paracomplex manifold $(M,\Omega_{\frak{C}})$ where the 2-form can be written as 
%$\Omega_{\frak{C}}=-\frac{e}{2}g_{jk}dx^i\wedge dy^i,$
%where $z^i=x^i+ey^i$.
%\end{lem}

In order to show that this manifold is symplectic it is sufficient to notice that the Hamiltonian discussed previously is associated to the following functional:

\begin{equation}\label{E:1}
\langle \mu, f\rangle=\int_{\tilde{\Omega}}f(\omega)\mu\{d\omega\},\end{equation}
where $f$ is a $\cF$-measurable function and $\mu$ is a dominated measure on the measurable space $(\tilde{\Omega},\cF)$. In the discrete case, this is given by: 

\[\langle \mu, f\rangle=\sum_{j=1}^m f^j\mu_j.\]

%Those $\cF$-measurable functions form not only a linear space but also an algebra. 

%%The functional appearing in~\eqref{E:1} can be identified to a Hamiltonian. 

We want to express the Hamiltonian for statistical manifolds, being Frobenius. From \cite{CoMa20,CoCoNen21} we have that the statistical manifolds (satisfying the Frobeniusity condition) have geometry of the Lie group of type $SO(1,n-1)$. The bilinear form for this group, is given by :
%\[|x_0|^2=\sum_{\mu,\nu=1}^{n-1} g^{\mu\nu}x_\mu x_{\nu},\]
%where $g^{\mu\nu}$ is the metric (which is trivial here).
%− c2dτ2 = ημνdxμdxν,
\[\kappa_1ds^2=\lambda_{\mu\nu} dz^{\mu}dz^{\nu},\]
where $\{\lambda_{\mu\nu} \}$ is a diagonal matrix $(1,1,1,-1)$ and $\kappa_1$ is a constant.



So, the Lagrangian written in terms of the tangent vector is given by: $\mathcal{L}=\frac{1}{2}C(\xi^\mu\xi_{\mu}-1)+ \kappa_2\xi^\mu A_{\mu}$
where $A_{\mu}$ corresponds to the Gauge Abelian field; $C$ and $\kappa_2$ are constants. 
The so-called ``momentum'' and ``force'' are derived from the Lagrangian, respectively as follows:
\[p_{\mu}=\frac{\partial \mathcal{L}}{\partial \xi^\mu}=\xi_{\mu}+\kappa_2A_{\mu},\]
\[f_{\mu}=\frac{\partial \mathcal{L}}{\partial z^\mu}=\xi^\mu\frac{\partial A_{\nu}}{\partial z^\mu}.\]

This allows to write the Hamiltonian using the Lagrangian view point for our case. In other words we have:
\[\mathcal{H}=\xi^\mu\frac{\partial\mathcal{L}}{\partial \xi^\mu}-\mathcal{L}=\xi^\mu p_{\mu}-\mathcal{L}.\]
%On the other side, this functional can be also linked to the Fisher metric, which corresponds to the metric tensor.\
So, in this way we show that our information geometry manifold has Hamiltonian structure.    
Finally, since the manifold under consideration is Frobenius, this implies it has torsionless and flatness properties. Therefore, by the above statement it forms an integrable system. Now, the existence of the Hamiltonian implies that this Frobenius manifold is symplectic. $\square$


%This Gauge Abelian field in stats manifold is related to the conditional probabilities
\smallskip 

We have thus ended the proof of the main theorem. In the next part, we discuss other implications of this on the geometry.  
\endinput
\section{}

Recall that the Riemannian manifold possesses a pair of dual torsionless flat connections. Then there exists a pair $(\theta,\eta)$ of dual coordinate systems such that $\theta$ is $\nabla$-affine and $\eta$ is $\nabla^*$-affine. By putting, 
\[\partial_i=\frac{\partial}{\partial\theta^i}\quad \partial^j=\frac{\partial}{\partial\eta_j},\]
where 
\[\langle \partial_i,\partial_j \rangle=g_{ij},\quad \langle \partial^i,\partial^j \rangle=g^{ij}. \]


Note that $g^{ij}$ is the inverse of $g_{ij}$ as raising and lowering operators for vector fields and that . Also, we have a pair of potential functions, which obey to the following equations $g_{ij}=\partial_i\partial_j\phi$ where $\phi$ is a potential function  and $g^{ij}= \partial^i\partial^j\psi$.  
 

\medskip 

By Mokhov, we have the following statement:

\begin{thm}[\cite{Mo09}] The function $\phi$ are solutions of the WDVV equation and generate the pair of operators (Lax operators, and include Hamiltonians).\end{thm}

In particular, this is statement is of interest when one considers the following. 


Recall from \cite{CoCoNen} that for $k$ be the field of real numbers. Let $S$ be the information geometry Frobenius manifold. The Gromov--Witten invariants for statistical manifolds (GWS) are given by the multi-linear maps:
 \[\tilde{Y}_n:S^{\otimes n}\to k.\] 

One can also write them as follows: \[\tilde{Y}_n\in \left(-\sum_{j}\beta^jX_j(\omega)\right)^{\otimes n}.\]

In particular, the Hamiltonian comes from the equation given by $\tilde{Y}_n$. 

The (GWS) invariants and the Hamiltonian appear as part of the potential function $\tilde{\bf \Phi}$, which is a Kullback--Liebler entropy function. 

One can write the relative entropy function:
\begin{equation}\label{E:3}\tilde{\bf \Phi}= ln \sum_{\omega\in\Omega} \exp{(-\sum_{j}\beta^jX_j(\omega))}.\end{equation}

Therefore, we state the following:
\begin{prop}
The entropy function $\tilde{\bf \Phi}$ of the statistical manifold relies on the Hmailtonian.
\end{prop}


[STREATER article. explicit  relation to Thermodynamics. Hamiltonian.]
\medskip 

Let us analyse this formula and show the existence of the Hamiltonian action structure in our case. Form \cite{CoMa20}, we know that the information geometry Frobenius manifold is a submanifold of the fifth Vinberg cone. 
The quadratic differential form on the cone $V$ that coincides with $d^2\ln\phi$ is any affine coordinate system defines the structure of a Riemannian space on $V$. In affine coordinate system the components of the metric tensor $g$ are given by the formula:
\[g_{ij}=\partial_{ij}\ln\phi.\] 
Given a point $x_0$ in the (Vinberg) cone $V$,  the tangent space to $V$ at $x_0$ is identified to a linear space $R$ and in it a multiplication operation $\circ$ is defined. In any affine coordinate system, this (commutative) multiplication is obtained by:

\[a\circ b=-\Gamma_{jk}^i(x_0)a^jb^k,\quad (a,b\in R)\]
  
For any automorphism $A$ of $V$, we have that the differential form $d^2\ln \phi$ is invariant under $A$ i.e.:

\[\ln\phi(Ax)=\ln\phi(x)-\ln det(A).\] 
Let us consider an arbitrary smooth $n$-dimensional submanifold in an $(n + m)$-dimensional pseudo-Euclidean space of some given signature $q$.
We suppose that the induced metric---from the ambient pseudo-Euclidean space---on this submanifold is nondegenerate (i.e. $det(g_{ij})\neq 0$ for some given coordinate system). 

In addition, we require those submanifolds to be flat, with zero torsion in pseudo-Euclidean spaces. In other words, we ask those manifolds to be torsionless with flat metrics.

%\cite{Ba20}

\subsection{Duality relation}

We have formerly proved in our article that, we have a Frobenius algebra structure on the tangent space to the stats manifold with vanishing curvature.
By Mokhov, we know that:

all Tangent submanifold are pseudo elliptic space have a Frobenius algebra on their tangent space and this forms a duality.

\medskip
\subsection{Hamiltonian}
We construct a Hamiltonian for a Frobenius algebra of rank 2. Let us take a point $P$ in the linear space (realization of a module over this algebra).
There exists a local coordinate system defined for this point. At this point, we attach a tangent vector. 
Affinor = matrix such that for each element of the algebra,  we have 

\[\{f\}=\begin{pmatrix} f_1^1 & f_1^2 \\ f_2^1 & f_2^2  \end{pmatrix}\]

